Domain Generalization through Audio-Visual Relative Norm Alignment in First Person Action Recognition

First person action recognition is becoming an increasingly researched area thanks to the rising popularity of wearable cameras. This is bringing to light cross-domain issues that are yet to be addressed in this context. Indeed, the information extracted from learned representations suffers from an intrinsic "environmental bias". This strongly affects the ability to generalize to unseen scenarios, limiting the application of current methods to real settings where labeled data are not available during training. In this work, we introduce the first domain generalization approach for egocentric activity recognition, by proposing a new audio-visual loss, called Relative Norm Alignment loss. It re-balances the contributions from the two modalities during training, over different domains, by aligning their feature norm representations. Our approach leads to strong results in domain generalization on both EPIC-Kitchens-55 and EPIC-Kitchens-100, as demonstrated by extensive experiments, and can be extended to work also on domain adaptation settings with competitive results.

==> latex/OldFiles/FPAR_RWorks.tex <==
\textbf{First Person Action Recognition.} The main first-person action recognition approaches proposed so far can be divided into two main groups. The first one exploits Long Short-Term Memory and variants \cite{Sudhakaran_2017_ICCV,sudhakaran2018attention,sudhakaran2019lsta,furnari2020rolling}, and the second leverages 3D convolutional kernels which jointly generate spatial-temporal features by sliding along the spatial and temporal dimensions \cite{singh2016first,tran2015learning,Wu_2019_CVPR,kapidis2019multitask}. Many methods have been also suggested that integrate RGB with motion information, i.e., Optical Flow, on multi-stream architectures \cite{carreira2017quo,10.5555/2968826.2968890,ma2016going, lu2019learning}, many of which are inherited from the third-person action recognition literature. 
Following architectures have focused on modelling longer temporal structure through consensus of predictions over time [TSM, TRM, TSN, TBN], or investigated several alternative approaches to fuse streams \cite{sudhakaran2019hierarchical,wangsymbiotic,Wu_2019_CVPR,zhou2018temporal}. However, although optical flow has proven to be a strong asset for the action recognition task, it is computationally expensive. As shown in \cite{Crasto_2019_CVPR},
the use of optical flow limits the application of several methods in online scenarios, pushing the community either towards single-stream architectures~\cite{zhao2019dance,Crasto_2019_CVPR,lee2018motion,sun2018optical,planamente2020joint}, or to investigate alternative modalities, e.g., audio information [CITA]. Although the audio modality has been proven to be robust in egocentric scenarios by \cite{Kazakos_2019_ICCV,cartas2019seeing}, this paper is the first that exploits it, jointly with its visual counterpart, in a cross-domain context. 

==> latex/OldFiles/IntroOld.tex <==
\section{Introduction}
\begin{centering}


\begin{figure}[t]

    \includegraphics[width=\linewidth]{latex/Img/teaser.pdf}
    \caption{
    %Egocentric action recognition comes with  a rich sound representation, due to the frequent hand-object interactions and the closeness of the sensor to the sound source. However, 
    The correlation between the distinctive sound of an action and its corresponding visual information is not always guaranteed across domains in egocentric action recognition. For instance, %in a clip where 
    the action \textit{cut} might produce or not a  characteristic sound depending on the object it involves, while %or the scene where it is performed. Likewise, 
    its visual appearance 
    %of the action 
    might vary significantly in different settings. By learning to combine effectively audio-visual information from multiple source domains, we are able to recognize first person activities across domains.}
%the information brought by the audio will be referred to only as background noise (and thus strictly domain dependent). Conversely, for the same action carried out with another object or in a different setting, the aural information might be highly informative and more robust to environmental changes. 


%first person activity recognition. 
    %%the appearance information (RGB) and the audio signal,
    %proved to obtain good results in the context of first person action recognition. %Our insight is based on the assumption that both these two kinds of data
    %Our insight is that both modalities might suffer from the domain shift due to the inevitable environmental bias, %but we believe that the heterogeneous nature of them could be reflected in different ways in which the domain shift problems affect them.  
    %Our insight is that both modalities might suffer in different manners from the domain shift imputable to the environmental bias affecting each dataset. Hence, finding an efficient way to merge the two information to let one overcome the downsides of the other is crucial to resolve such issue.
%Hence, improving the cooperation between the two could help one modality to overcome the problem, introduced by the domain shift of the other, in a complementary way.
\label{fig:teaser}

\end{figure}
\end{centering}

%Egocentric vision plays a central role in a wide range of applications, such as human-computer interaction or human assistance. The recent release of the EPIC-Kitchen large-scale dataset   is achieving more and more interest by the research community, especially 


First Person Action Recognition is rapidly attracting the interest of the research community~\cite{sudhakaran2018attention,sudhakaran2019lsta,furnari2020rolling,Kazakos_2019_ICCV,ghadiyaram2019large,Wu_2019_CVPR}, both for the significant challenges it presents and for its central role in real-world egocentric vision applications, from wearable sport cameras to  human-robot interaction or human assistance. 
Although leveraging over advances in third person activity classification has brought  significant progress in this field, the intrinsic positioning of sensors in egocentric vision creates unique opportunities  and challenges. On one side, having the audio sensors intrinsically close to the performed actions means that high quality auditory information is available for recognizing activities. This is in contrast with third person settings, where actions usually happen far away from the recording sensors, or there might be other overlapping sound sources. %and hence audio is seldom used. 
On the other side, in egocentric vision the recording equipment is worn by the observer and it moves around with her. Hence, there is a far higher degree of changes in illumination, viewpoint and environment compared to a fixed third person camera. This in turn calls for  approaches able to deal robustly with varying visual domains at test time, with little (if none) ability to forecast such domain changes. For instance, the action ``cut" presents several audio-visual differences across domains: cutting boards will differ in their visual and auditory imprints (i.e. wooden cutting board vs plastic one), various kinds of edibles might be cut, and so forth (figure~\ref{fig:teaser}).

%as we can see in Figure \ref{fig:teaser}\chiara{, the action ``cut" presents several differences across domains, both visual (cutting boards differs in their appearance) and auditive (the woody cutting board will produce a sound which is different from the plastic one).}
%\chiara{Moreover, the correlation between the characteristic sound of an action and its corresponded visual information are not always guaranteed for all the videos. For instance, in a clip where the action \textit{take} does not produce any characteristic sound, %because of the object it involves, or the setting where it is performed, 
%the information brought by the audio will be referred to only as background noise (and thus strictly domain dependent). Conversely, for the same action carried out with another object or in a different setting, the aural information might be highly informative and more robust to environmental changes.} 
 %\babs{provare a mescolare/descrivere un po' il teaser qui, come esempio per far capire bene}
    

%A key opportunity, seldom used in this context, is the availability of auditory information for recognizing manipulation activities: while in third person settings actions might be performed too far away from the recording sensors, or there might be other overlapping sound sources, in first person action recognition the manipulation activities do happen intrinsically close to the audio recording, making it possible to exploit this modality in conjunction with RGB data. 
%Conversely, as the recording equipment is worn by the observer, it moves around with her, hence experiencing a far higher degree of changes in illumination, viewpoint and environment compared to a fixed third person camera.   

%\mirco{Add importance of Audio}

The recent release of the EPIC-Kitchen large-scale dataset \cite{damen2018scaling} has given a very significant boost to the research activities in this field, offering the possibility to study people’s daily actions from a unique point of view while at the same time confirming the distinctive features of egocentric vision highlighted above. The collection of this dataset consists in the segmentation of long untrimmed audio-visual recordings, representing people’s daily activities recorded in the same kitchen. This process results in a huge number of sample clips containing a large variety of action classes, which are however captured in a limited number of environments. This intrinsic unbalance causes the so called \textit{environmental bias}, meaning that the learned action representations are strictly dependent on the surroundings, and thus hardly able to generalize to videos recorded in different conditions \cite{torralba2011unbiased}. In general, this problem is referred to in the literature as \textit{domain shift}, meaning that a model trained on a source labelled dataset cannot generalize well on unseen data, called target. 


Recently, \cite{Munro_2020_CVPR} addressed this issue %for fine-grained AR 
by reducing the problem to an unsupervised domain adaptation (UDA) setting, where an unlabeled set of trimmed samples from the target is available during training. However, the UDA scenario is not always  realistic, because the target domain might not be known a priori or because it might be costly (or plainly impossible) to access target data at training time. 

In this paper we argue that the true challenge is to learn a representation %able to extract a knowledge from data which is transferrable 
able to generalize to any unseen domain, regardless of the possibility to access target data at training time. %This means developing a method general enough to deal with cross-domain settings regardless of the availability of target data at training time.
%to work both on UDA and Domain Generalization (DG) 
%\cite{pmlr-v28-muandet13}. %, the extreme case where target data are not accessible at training time.
%The considerations above motivate us to analyze the problematics of this problem, known as domain generalization (DG),rained context. 
Inspired by the idea of exploiting the multi-modal nature of videos  \cite{Munro_2020_CVPR} and by the availability of high quality audio-visual data, we propose the first egocentric Domain Generalization (DG) architecture that aligns different domains by learning a shared audio-visual representation, hence leveraging over the complementary nature of these two modalities.
%method which leverages over the complementary nature of visual and audio information. 
We start by observing that %first person action recognition intrinsically comes with rich sound information, due to the strong hand-object interactions and the closeness of the sensors to the sound source. The use of auditory information could be a good workaround for the problems which arise from the use of wearable devices, in that it is not sensitive to the ego-motion and it is not limited by the field of view of the camera.  Moreover, our idea is that, 
since the audio and visual modalities come from different sources, they suffer from a domain shift of different nature.
%the domain-shift they suffer from is not of the same nature.   
Motivated by this consideration, we propose a new cross-modal loss function, which we call \textit{Relative Norm Alignment loss}, that operates on the relative features norm of the two modalities, on different domain sources, acting on their magnitude. Our loss improves the cooperation between the audio and visual channels, effectively aligning different audio-visual domains by learning a new shared representation. Although our approach has been designed for the domain generalization setting, it can be extended easily to the domain adaptation scenario.
%which results in a stronger ability  to overcome the domain shift. 
Extensive experiments show that our approach leads to strong results  both in UDA and DG settings. We are not aware of previous works dealing with domain generalization in first person activity recognition.  %of the other in a complementary way.
%\mirco{The focus should be on DG}

To  summarize,  our  contributions  are  the  following: 
\begin{itemize}
   % \item  we present the first domain generalization deep architecture in first person action recognition that learns a shared cross-modal feature representation from audio-visual data; 
    \item we propose a new cross-modal audio-visual loss, the Relative Norm Alignment loss, that progressively aligns the relative feature norms of the two modalities from various source data, resulting in domain-invariant audio-visual features;
    \item  we present a new benchmark for %both single-source and 
    multi-source domain generalization in first person videos and extensively validate our method on both DG and UDA scenarios, achieving competitive results compared to previous works.
   % , which, to the best of our knowledge, no prior work has explored yet;
%    \vspace{-7pt}
%    \item we validate the effectiveness of our method on both DG and UDA scenarios, 
 %   \vspace{-7pt}
%
  %  \item  we empirically bring to light a
   % problem related to the heterogenous nature of audio and visual modalities, which causes an unbalance preventing the two modalities to correctly cooperate;
\end{itemize}




%Egocentric vision plays a central role in a wide range of applications, such as domestic or industrial robots. The camera is mounted onto a subject that is constantly moving, paving the way for new challenges which are increasingly attracting the attention of the community. In this context, fine-grained action recognition is the task of identifying the action being performed, along with the involved object. To analyze this problem in more depth, a useful tool is the largest dataset currently available \cite{damen2018scaling} on actions in first person, %Currently, the largest available dataset in this field is EPIC-Kitchens \cite{damen2018scaling}, 
%where a multitude of activities in various kitchens is recorded using a GoPro fixed on the head of the actor. From the numerous challenges posed by the authors of the dataset, it emerged that the community is focusing on achieving better performances in a single-domain context by developing more sophisticated architectures. Nevertheless, the non-negligible domain shift issue induced by different data distributions of training and test data%, i.e. multi-domain context, 
%has not been adequately addressed yet in this scenario. In fact, when training a model using data coming from a certain environment and deploying it on an unseen one, the performance are adversely affected.

%A solution is to perform unsupervised domain adaptation (UDA), that is training the model using both labeled data from an environment (\textit{source domain}), and unlabeled samples from a new one (\textit{target domain}). Despite the advancements made in third person video UDA to tackle this problem \cite{videoda-chen2019temporal,videoda-choi2020unsupervised,videoda-Jamal2018DeepDA}, only one work \cite{Munro_2020_CVPR} does it in first person with the addition of a supplementary modality, i.e. flow frames. Indeed, multi-modality has proven to be helpful for video DA \cite{}, but obtaining the commonly used additional flow modality is computationally costly \cite{}. The same cannot be said for audio, since in videos it freely comes paired with the RGB frames, which is why it is being employed more and more as added modality. When summed to visual modalities, aural signals demonstrated to be an effective modality to supply complementary information in fine-grained first person action recognition \cite{Kazakos_2019_ICCV}, as well as in other third person tasks \cite{}. 




%Sadly, UDA is not always applicable in real applications because the target domain might not be known a priori, so data from that distribution is not available at training time. This shifts the problem into the more complicated domain generalization (DG) setting, which differs from UDA in that target data is not seen at all at train time. Inspired by the findings of \cite{Kazakos_2019_ICCV}, we employ the additional auditive modality in a new way inside the DG scenario. We observe that, when fusing audio-visual embeddings, the contribution of each modality is not balanced due to a strong imbalance among the respective feature norms, leading to non-optimal performance. We therefore propose a cross-modal loss that aims at readjusting the norms, and thus, the contribution of each modality, by enforcing the ratio between the two to be equal to 1 (as shown in Figure 1). Moreover, we demonstrate how less relevant features are suppressed in favor of more important ones while solving this task.

%To summarize, our contributions are the following(da rivedere una volta conclusi gli experiments, inseriti solo dei placeholders temporaneamente):




==> latex/OldFiles/Method.tex <==
%\section{Relative Norm Alignment}\label{sec:preliminaries}
\section{ Cross-Domain Audio-Visual RNA-Net} \label{RNA-NET}


This section shows how \mylossRna %Relative Norm Alignment (RNA) 
 can be effectively used in a very simple audio-visual deep network for cross-domain first person action recognition. The network, shown in Figure \ref{fig:architecture}, inputs audio and visual information in two separate branches. After a separate convolution-based feature extraction step, the \mylossRna loss learns how to combine the two modalities, leading to a significant generalization across-domains, in both the domain generalization (DG) and unsupervised domain adaptation (UDA) settings. Below we describe in more details how the net works in both settings.
\subsection{Problem Statement}
Given one or more source domains $\{\mathcal{S}_1,...,\mathcal{S}_k\}$, where each $\mathcal{S}={\{(x^s_i,y^s_i)\}}^{N_s}_{i=1}$ is composed of $N_s$ source samples with label space $Y^s$ known, our goal is to learn a model representation able to perform well on a target domain $\mathcal{T}={\{x^t_i\}}^{N_t}_{i=1}$ of $N_t$ target samples whose label space $Y^t$ is unknown. Our two main assumptions are that the distributions of all the domains are different, \ie $\mathcal{D}_{s,i} \neq \mathcal{D}_t$ $\land$ $\mathcal{D}_{s,i} \neq \mathcal{D}_{s,j}$, with $i \neq j$, $i,j=1,...,k$, and that the label space is shared, $\mathcal{C}_{s,i} = \mathcal{C}_t$, $i=1,...,k$. In this work we consider two different scenarios:
%\begin{itemize}

\noindent
{\textbf{Domain Generalization (DG)}},
where at training time the model can access one or more fully labeled source datasets $\mathcal{S}_1,...,\mathcal{S}_m$, but no information is available about the target domain $\mathcal{T}$.

\noindent
{\textbf{Unsupervised Domain Adaptation (UDA)}}, where at training time it is possible to access a set of unlabeled target samples belonging to the target domain $\mathcal{T}$, jointly with one fully labeled source domain $\mathcal{S}$.

%Under this setting, during training time, in addition to one fully labeled source domain $\mathcal{S}$, a set of unlabeled target samples belonging to the target domain $\mathcal{T}$ is available. 


%During training time, the model disposes of one or more fully source labeled datasets $\mathcal{S}_1,...,\mathcal{S}_m$, but no information is available about the target domain  $\mathcal{T}$. Thus, the goal is to build a model able to generalize well on unseen domains. 
%\end{itemize}
\noindent
For both scenarios, the ultimate goal is to learn a model able to generalize well on the target data. 


\textbf{Multi-Modal Approach.} Our goal is to investigate how using multi-modal signals from source and target data affects the ability of a first-person action classification net to generalize across domains.
%We are interested in a setting where the source and target data consist of multi-modal signals, with the aim to investigate how this affects the ability of a first-person action classification architecture to generalize across domains.
Specifically, given
a multi-modal input $X=(X^1,...,X^M)$, where $X^m=(x^m_1,...x^m_{N_m})$ is the set of all $N_m$ samples of the $m$-th modality, we use a separate feature extractor $F^m$ for  $X^m$%corresponding to the $m$-th modality
, and we employ all the $f_m=F^m(x^m_i)$ corresponding features, encoding information from multiple channels,  during the learning process. 
%We introduce this notation for clarity, as it will be used in the next section.



\begin{figure*}[t]
    \centering
    %\includegraphics[width=\linewidth]{latex/Img/Net.pdf}
     %\includegraphics[width=\linewidth]{latex/Img/net4.png}
     %\includegraphics[width=\linewidth]{latex/Img/Net7.png}
    \includegraphics[width=\linewidth]{latex/Img/net_onlyDG.png}
    
    \caption{\textbf{RNA-Net.} Labeled \textcolor{OliveGreen}{source visual} $x^v_{s,i}$ and \textcolor{RoyalBlue}{source audio} $x^a_{s,i}$ inputs are fed to the respective feature extractors $F^v$ and $F^a$.  \textcolor{Orange}{Unlabeled target} data of any modality ($x^m_{t,i}$) is seen at training time only in UDA setting, and not in DG. Our $\mathcal{L}_{RNA}$ operates at feature-level by balancing the relative feature norms of the two modalities. The action classifiers $G^v$ and $G^a$ are trained with standard cross-entropy loss $\mathcal{L}_{ce}$. At inference time, multi-modal target data is used for classification.
    }
    
    %\textbf{RNA-Net.} \textcolor{OliveGreen}{Source} visual $x^v_{s,i}$ and \textcolor{Orange}{target} visual inputs $x^v_{t,i}$ are fed to the visual stream. Conversely, the \textcolor{RoyalBlue}{source} audio input $x^a_{s,i}$ and \textcolor{Orange}{target} audio input $x^a_{t,i}$, are fed to the audio stream. Feature extractors are separate for each modality, and shared for both source and target data. Our $\mathcal{L}_{RNA}$ operates at feature-level by balancing the relative feature norms of the two modalities. The audio and visual classifiers are trained with standard cross-entropy $\mathcal{L}_{entropy}$ using source data. During inference, multi-modal target data are used for classification. Note that in the DG scenario target data is not available during training.   }
    
    \label{fig:architecture}
    \vspace{-13 pt}
\end{figure*}

\subsection{AV-RNA-Net for Domain Generalization}
\label{sec:dg}

In a cross-modal context, the input comes from one or more source domains $\mathcal{S}_k=(\mathcal{S}^v,\mathcal{S}^a)$. Under the DG setting, the target is not available during training (see Section~\ref{sec:preliminaries}). % For simplicity, we denote with $X^m=(\mathcal{S}_m, \mathcal{T}_m)$ the set of inputs for the $m$-th modality, where $x^m=x^m_s$ while training, while $x^m=(x^m_s,x^m_t)$ is a tuple composed by both a source and target sample at inference time. 
As shown in Figure \ref{fig:architecture}, each input modality is fed to a separate feature extractor, $F^v$ and $F^a$ respectively. The resulting features $f_v=F^v(x^v_i)$ and $f_a=F^a(x^a_i)$ are then passed to separate classifiers $G^v$ and $G^a$, whose outputs correspond to distinct score predictions (one for each modality). The two are combined with a \textit{late fusion} approach and used to obtain a final prediction $P(x)$ (please refer to Section \ref{sec:experimental} for more details). Our loss \mylossRna operates at feature-level before the final classification, acting as a bridge between the two modalities and encouraging a balance between the respective contributions.
\mirco{The RNA-Net is trained minimizing the total loss defined as}
\begin{equation}\label{eq:total_loss}
    \mathcal{L}= \mathcal{L}_C + \lambda \mathcal{L}_{RNA},
\end{equation}

where the $ \mathcal{L}_C $ is defined as a cross-entropy and $\lambda$ indicates the weight given to our loss $ \mathcal{L}_{RNA}$ during training. 

%Following previous works on multi-modal action recognition \cite{Munro_2020_CVPR, quo_vadis, tsn, trr, tsm}, we use a multi-stream structure, i.e., a separate stream for the visual and audio input, a


\subsection{Relative Norm Alignment Loss} \label{sec:rna_loss}
Starting from the above considerations, our intuition is that a large misalignment at feature-norm level negatively affects the learning process by causing an unbalance between the contributions brought by each modality, which therefore degrades the classification performance.
% Considering the dot product $<f_v, f_a>$, defined as
%\begin{equation}
%\label{formula:dot_product}
%    <f_v, f_a>= {\lVert f_v \rVert}_2 {\lVert f_a \rVert}_2 \cos{\theta} ,
%\end{equation}
%our approach involves the first two terms of Equation \ref{formula:dot_product}, imposing a relative alignment between them. \\ 
To formalize the norm misalignment, we denote with $h(x^m_i)=({\lVert{ \cdot }\rVert}_2 \circ f_m)(x^m_i)$ the $L_2$-norm of the features $f_m$ of the $m$-th modality. To ease the readiness of the next steps, we introduce a term $\delta(h(x^v_i),h(x^a_i))$ to characterize the \textit{mean-feature-norm distance} between the norms of $f_v$ and $f_a$. We define the discrepancy $\delta$ between the two modality norms by means of a simple scalar distance, formulated as 
%The discrepancy between their norms, i.e., $ h(x^v_i)$ and $h(x^a_i)$, is measured by a \textit{mean-feature-norm distance} term $\delta$, defined as:
\begin{equation}
    \delta(h(x^v_i),h(x^a_i))=\lvert{\frac{1}{N}\sum_{x^v_i \in \mathcal{X}^v}h(x^v_i)-\frac{1}{N}\sum_{x^a_i \in \mathcal{X}^a} h(x^a_i)\rvert}
\end{equation} 
where $N=|\mathcal{X}^v|=|\mathcal{X}^a|$ denotes the number of the samples for each modality. Figure \ref{fig:OurLoss} illustrates the norm $h(x^v_i)$ of the $i$-th visual sample and $h(x^a_i)$ of the $i$-th audio sample, by means of segments of different lengths arranged in a radial pattern. The mean feature norm $\frac{1}{N}\sum_{x^k_i \in \mathcal{X}^k}h(x^k_i)$ of the $k$-{th} modality is represented by the radius of the two circumferences, and $\delta$ is represented as their differences.
%\barbara{ho modificato l'ultima frase per renderla specifica del cross-modal, please check!} 


To this purpose, we propose a relative norm alignment (RNA) loss function is defined as
\begin{equation}\label{formula:rna}
    \mathcal{L}_{RNA}=\left(\frac{\EX[h(X^v)]}{\EX[h(X^a)]} - 1\right)^2,
\end{equation}
where we define $\EX[h(X^m)]=\frac{1}{N}\sum_{x^m_i \in \mathcal{X}^m}h(x^m_i)$ for the $m$-th modality and $N$ denotes the number of samples of the set $\mathcal{X}^m=\{x^m_1,...,x^m_N\}$. This dividend/divisor structure is used to encourage a relative adjustment between the norm of the two modalities, enhancing an \textit{optimal equilibrium} between the two embeddings.

Conceptually, aligning the two modality norms is the same to impose a more  ``hard" constraint and align them to a constant value $k$ (\textit{Hard Norm Alignment}), as in the following: 
\begin{equation}
    \mathcal{L}_{HNA}=\left(\EX[h(X^m)] - k\right)^2,
\end{equation}

where $k$ is the same for both modalities. 
However, we formulated the  $\mathcal{L}_{RNA}$ specifically for avoiding having the introduction of 
a fixed $k$ hyper-parameter, for two main reasons.
First, ideally each domain would require its own ``optimal" $k$ which indeed, having to be fixed, could lead to sub-optimal solutions. Secondly, a strong discrepancy between the value of $k$ and the range where the norms vary would reflect in an high norm alignment loss, potentially affecting negatively the learning process of the primary action classification task. To overcome this limit, an accurate tuning of the weights of the loss would be required, which would have increased the sensibility of the network to loss weights \cite{kendall2018multi}.
With our loss we avoid introducing a fixed $k$ while guiding the convergence of the network towards the optimal balance between the two norm distributions. 

Moreover, while the alignment could be solved through a ``subtraction" between the two modality norms (forcing their difference to be zero), %is conceptually the same of ``ratio", 
the choice of a ``ratio" structure ensures the loss to be in the 
range $(0,1]$, starting from the modality with higher norm as a dividend. The resulting loss is less sensitive to loss weight variations among domains.


When minimizing \mylossRna, the network can either increase the divisor $(f_v \nearrow)$ or decrease the dividend $(f_a \searrow)$, leading to three potential main benefits.
\begin{figure}[t]
    \centering
    %\includegraphics[width=1\linewidth]{latex/Img/diagram-20210309.png}
    \includegraphics[width=1\linewidth]{latex/Img/RNA_Idea8.png}

    %\includegraphics[width=1\linewidth]{latex/Img/NormDistribution.pdf}
    \caption{\textbf{Feature Distribution Adjustment.} (a) shows the distribution of \textcolor{OliveGreen}{visual} and \textcolor{RoyalBlue}{audio} features. We see that, without any form of alignment, audio features are predominant over visual ones, which could ultimately lead to a loss of information. By minimizing $\mathcal{L}_{RNA}$, several possible scenarios can occur, displayed second row. In this scenario, the range where the feature norms vary is the same, making the informative content of the two distributions comparable with each other. This lets the loss learn from data when it is more convenient to align them (\textit{Alignment} or \textit{Euclidean loss}) or when it is better to preserve their peculiarities (\textit{Orthogonality loss}).
    }
    \label{fig:OurLoss}
    \vspace{-0.2cm}
\end{figure}
%\begin{enumerate}[itemsep=1pt, topsep=0pt, partopsep=0pt]

    \textbf{Audio-Visual Re-balance.} Since $\EX[h(X^v)]$ and $\EX[h(X^a)]$ tend to the same value, features norm ranges are encouraged to be comparable, preventing one modality to incorrectly drown out the other (refer to Section \ref{norm_unbalance}). 
    Moreover, by imposing a constraint on RNA while solving the main task we increase the norm of the discriminative features when arising the norm, while we %forcing the network to reduce 
reduce the norm of those non-discriminative when decreasing it. The \textit{smaller-norm-less-informative} assumption \cite{ye2018rethinking} 
suggests that 
features with smaller norms are less informative at inference time.  
    
\textbf{Audio-Visual Complementary.} The correlation between the characteristic sound of an action and its corresponded visual information are not always guaranteed for all the videos. Therefore they could exist some clips where one of the two modality contains only information about the domain shift (environment bias or background noise). In these situations an alignment constraint ($\theta \rightarrow 0$) could be potentially dangerous, in particular to exploit the complementary of the two modalities in across domain scenario.
Starting from these consideration, we believe that they exist some situations where the network could benefit from exploiting the heterogeneity of the data to overcome the difficulties introduced by domain shift. In this case, a loss that minimizes the overlapping information about the two modalities by encouraging to properly exploit the unique characteristics about the two, could be potentially better ($\theta \rightarrow \pm 90$).

Our intuition is that a loss should give the possibility at the feature distributions to preserve their modality-specific features when one modality is weak or contain only domain-information and align them when both are correlated with action. In fact, by not constraining the angular distance $\theta$ between the two modality representations, we do not strictly enforce an alignment of two (when non-necessary) or an orthogonality, letting the network to find itself the better angle for the main task. 

\par{\textbf{Why should \mylossRna help to generalize?}} Our loss \mylossRna rises the generalization ability of the network for two main reasons. First, by self-reweighting the two modalities contribution during training, the classifier has the chance to rank such contributions according to their real relevance, thus avoiding to be fooled by the natural unbalance due to their intrinsic heterogeneity. This is helpful especially in a multi-source setting, as it ensures uniformity not only across modalities, but also across data from different sources. Secondly, by undirectly minimizing the norm of the feature activations, our loss sets a limit to the learner feature encoding, and thus it forces it to only learn the discriminative information. As a consequence, the classifier can learn to ignore information which is strictly domain-specific, distilling the most useful and transferable features.

%\subsection{Overview}
%Our goal is to learn a model representation which, using video clips of the source domain and their corresponding sound, is able to predict well over 


%Learning Framework Cross-modal learning enclose all those methods which leverage over the knowledge from multiple modalities to produce the final classification. Given a multi-modal input $X=(X^1,...,X^M)$, where $X^m=(x^m_1,...x^m_N)$ is the set of all samples of modality $m$-th, each 


%\subsection{Baseline}
%In this section we present an overview about our baseline architecture and how it combines audio-visual modalities. Following previous works on multi-modal action recognition [cita!], we used a multi-stream architecture. Given a multi-modal input $X=(X^1,...,X^M)$, where $X^m=(x^m_1,...x^m_N)$, is the set of all samples of modality $m$-th, we used a separate feature extractor $F^m$ for the input $X^m$ corresponding to the $m$-th modality. The resulting features $F^m(x^m)$ are fed to a separate classifier $G^m$, whose outputs correspond to separate score predictions (one for each modality). The sum of the two is passed to standard \textit{cross entropy loss} to train the network obtain a final prediction $P(x)$. In this work, we consider $M=2$ modalities, i.e., RGB clip (visual stream) and audio signal (audio stream). To simplify the notations for more clarity, we use the notation $x^v_i \in \mathbb{R}^{T\times H\times W}$ to denote a visual sample $i$-th, and $x^a_i \in \mathbb{R}^{T\times H\times W}$ to denote the $i$-th audio sample, represented as a spectrogram image. Moreover, we indicate with $f_v=F^v(x^v_i)$ and $f_a=F^a(x^a_i)$ the features extracted from the visual and audio stream respectively.


%Our setting is a {Cross-Domain Multi-Modal Framework}, which proposes to increase the model generalization ability by leveraging over the knowledge from multiple modalities.




\subsection{Audio-Visual Alignment} \label{angular_losses}
\label{sec:assumptions}

Let us consider a multi-modal framework characterized by $M=2$ modalities, specifically RGB clips and audio signals. We indicate with $f_v=F^v(x^v_i)$ and $f_a=F^a(x^a_i)$ the features encoding the visual and audio information, respectively (details about the feature extractor modules are given in Section \ref{RNA-NET}).
%Let us consider a multi-modal framework characterized by $M=2$ modalities, specifically RGB clips and audio signals. We indicate with $f_v=F^v(x^v_i)$ and $f_a=F^a(x^a_i)$ the features encoding the visual and audio information, respectively (details about the feature extractor modules are given in Section \ref{RNA-NET}). %\chiara{We introduce a term $\delta(h(x^v_i),h(x^a_i))$ to characterize the \textit{mean-feature-norm distance} between the norms of $f_v$ and $f_a$, which we indicate as $h(x^v_i)$ and $h(x^a_i)$ respectively. We thus define the discrepancy $\delta$ between the two modality norms by means of a simple scalar distance, formulated as  }
%The discrepancy between their norms, i.e., $ h(x^v_i)$ and $h(x^a_i)$, is measured by a \textit{mean-feature-norm distance} term $\delta$, defined as:
%\begin{equation}
%    \delta(h(x^v_i),h(x^a_i))=\lvert{\frac{1}{N}\sum_{x^v_i \in \mathcal{X}^v}h(x^v_i)-\frac{1}{N}\sum_{x^a_i \in \mathcal{X}^a} h(x^a_i)\rvert}
%\end{equation} 
%where $N=|\mathcal{X}^v|=|\mathcal{X}^a|$ denotes the number of the samples for each modality. Figure \ref{fig:Feat_Norm} \chiara{illustrates the norm $h(x^v_i)$ of the $i$-th visual sample and $h(x^a_i)$ of the $i$-th audio sample, by means of segments of different lengths arranged in a radial pattern. The mean feature norm $\frac{1}{N}\sum_{x^k_i \in \mathcal{X}^k}h(x^k_i)$ of the $k$-{th} modality is represented by the radius of the two circumferences, $R_v$ and $R_a$ respectively, and $\delta$ is represented as $\left| R_a - R_v \right|$.}
%\barbara{ho modificato l'ultima frase per renderla specifica del cross-modal, please check!} 
%\chiara{Our intuition is that a large $\delta$, i.e., a misalignment at feature-norm level, negatively affects the learning process by causing an unbalance between the contributions brought by each modality, which therefore degrades the classification performance.}
%Figure \ref{fig:Feat_Norm} illustrates the feature norms of the two modalities and the $\delta$ between the two.
%\barbara{Sarebbe importante qui fare piu' esplicitamente riferimento alla figura e a quello che rappresenta; parallelamente, forse si potrebbe aggiungere alla figura $\delta$? }
It has been shown in the literature that aligning audio and visual information by solving synchronization tasks~\cite{look_listen_learn,multisensory_owens, cooperative_torresani,objects_that_sound,afourasself} leads to representations that facilitate a number of audio-visual downstream tasks, including action recognition. Such approaches enforce feature alignment by means of Euclidean \cite{objects_that_sound} or similarity-based losses~\cite{afourasself}, whose objective is to embed audio and visual inputs into a shared representation space. 
Our intuition is that the optimization of these loss functions could, to some extent, limit action recognition networks when dealing with cross-modal scenarios. 
%In literature, it has been shown that the alignment between audio and visual information \chiara{by solving a synchronization task} leads to good action recognition results \cite{look_listen_learn,multisensory_owens, cooperative_torresani,objects_that_sound,afourasself}.  by means of Euclidean and similarity-based losses, whose objective is to embed the audio and visual inputs into a shared space.
%in exploiting the cross-modal potentiality. 

Let us consider the standard \textit{scalar product} between $f_v$ and $f_a$ defined as 

\begin{equation}
<f_v, f_a>= \lVert{f_v} \rVert_2 \lVert{f_a} \rVert_2 \cos(\theta)  ,
\end{equation}
where $\theta$ is the angle between the two modality feature vectors. When minimizing the Euclidean distance, both the magnitude ($\lVert{f_v} \rVert_2$ and $\lVert{f_a} \rVert_2$) and angular ($\cos(\theta)$) components are involved. Instead, when minimizing similarity-based losses, a constraint on the angular distance $\cos(\theta)$ between the two embeddings is imposed; indeed, the magnitude of the embedding does not play any direct role in the measure. We call these losses acting on the angular distance \textit{angular losses}, and we give an overview of their effect in Figure \ref{fig:OurLoss}.
%\chiara{Losses which aim to minimize the cosine similarity between $f_v$ and $f_a$ act on the angular distance $cos(\theta)$ between the two embeddings; }
%These losses mainly use the angular distance $\theta$ between the two embeddings, %defined as $\theta=arccos(\frac{\mathbf{f}_v\cdot \mathbf{f}_a}{\lVert{f_v}\rVert_2\lVert{f_a}\rVert_2})$.%, rather than acting on the magnitude of audio and visual norms. 


Angular losses indeed capable of aligning the two representations %(Figure \ref{fig:OurLoss}-b) 
but they struggle to exploit the modality-specific characteristics of the two streams. 
%As such, they induce a common representation, but limits the potential of the modality-specific ones, forcing an overlapping between two information which are not necessarily coherent. 
In other words, when using an angular loss we impose %on the network %is induced with 
the prior that what is significant for the visual stream is significant also for the audio stream, but this might not be true in practice, especially when training and test data come from different distributions. 
%\begin{figure}[t]
 %   \centering
  % \includegraphics[width=1\linewidth]{latex/Img/Idea.pdf}
%    \caption{\textbf{Relative Norm Alignment.} The norm $h(x^v_i)$ of the $i$-th \textcolor{OliveGreen}{visual} sample (top-left) and $h(x^a_i)$ of the $i$-th \textcolor{RoyalBlue}{audio} sample (top-right) are represented, by means of segments of different lengths. The radius of the two circumferences represents the mean feature norm of the two modalities, and $\delta$ their discrepancy. 
%    By minimizing $\delta$, audio and visual feature norms are induced to be the same, as shown at the bottom.
    %Through our $\mathcal{L}_{RNA}$, audio and visual features norms are aligned by inducing them to have the same value, i.e., same radius, while reducing the term $\delta$ to zero (Bottom).   }
%    }
%    \label{fig:Feat_Norm}
 %   \vspace{-0.2cm}
%\end{figure}

\chiara{Collegamento tra angolo e alllineare cose diverse}

For instance, in a clip where the action \textit{take} does not produce any characteristic sound, %because of the object it involves, or the setting where it is performed, 
the information brought by the audio will be referred to only as background noise (and strictly domain dependent). Conversely, for the same action carried out with another object or in a different setting, the aural information might be highly informative and more robust to environmental changes.%, which are usually due to appearance. 

%We show below with a set of experiments (Section \ref{sec:experimental}, Figure \ref{fig:PlotAccNorm}) that a large $\delta$, i.e., a misalignment at feature-norm level, negatively affects the learning process by causing an unbalance between the contributions brought by each modality, which therefore degrades the classification performance. 
Motivated by the  considerations above, we propose a new cross-modal loss function, which as opposed to losses acting on the angular distance,  operates on their magnitude. This intuitively results in more freedom to preserve the modality-specific features. %(see Figures \ref{fig:OurLoss}-b-c). 
We expect this to be important in cross-domain scenarios. 



 





%we say $f(a_i)$ is \textit{orthogonal} to $f(v_i)$, i.e., $f(a_i)$ $\perp$ $f(v_i)$, if their modality-specific information is complementary. Instead, we say $f(a_i)$ is \textit{parallel} to $f(v_i)$, i.e., $f(a_i)$ $\parallel$ $f(v_i)$, if the information is shared between the two. 

%We define $g(v_i)=({\lVert{ \cdot }\rVert}_2 \circ f(a_i))(v_i)$ and $g(a_i)=({\lVert{ \cdot }\rVert}_2 \circ f(a_i))(a_i)$ as the $L_2$-norms of the features extracted from the visual and audio streams respectively. We characterize their distance by defining the mean-feature-norm discrepancy between them, defined as:

%\begin{equation}
%    \delta(g(v_i),g(v_i))=\frac{1}{n_v}\sum_{v_i \in \mathcal{M}_v}g(v_i)-\frac{1}{n_a}\sum_{a_i \in \mathcal{M}_a} g(a_i) 
%\end{equation}
%We observe that a large $\delta$ corresponds to a misalignment between the two modalities which is revealed as one modality drowning out the other, preventing the network to exploit their orthogonality or parallelism. 

%This has as a side-effect a strong unbalance between the final predictions of the two, preventing them to cooperate to the final classification.


%\mirco{Add  training UNBALANCE, come se fosse un secondo problema}

\subsection{Norm Unbalance} \label{norm_unbalance}

Another important research question is: \textit{what is the best way to combine data from different modalities?} \cite{}.


Multiple works in the literature proposed approaches to learn a way to combine them in efficient ways in order to exploit their peculiarities \cite{}, trying to answer to questions regarding \textit{when} and \textit{how} combing them. 

In this work we investigate the reason \textit{why} the network struggle to deal with modalities of different nature. We believe that the intrinsic differences in the modality representations learned by each stream cause the network not being able to measure and understand which modality is informative and should rely on in the final prediction, and which one is useless. In fact, the two modalities do not share the same representation space and thus the classifier find hard to be aware of the right \textit{amount} of information brought by the two. 


%In this work we investigate the reason \textit{why} the network struggle to deal with modalities of different nature. We believe that the intrinsic differences in the modality representations learned by each stream cause the network not being able to to be aware of the right \textit{amount} of information brought by the two, and thus not being able to understand which one should rely on in the final prediction. %In fact, the two modalities do not share the same representation space and thus the classifier find hard  



Starting from the above considerations, our objective aims to re-balance the modality contributions of the two in order to easily make them comparable. To this purpose, the \textit{smaller-norm-less-informative} assumption \cite{ye2018rethinking} suggests us to use the norms to measure the \textit{amount} of information. In particular, the representations with smaller norms play a less informative role during inference, causing the modality with the larger feature norms to drown out the other during training. 
From our analysis emerged that different representation spaces correspond to different norm ranges, confirming the unbalanced contribution between the two modalities since the beginning of the training process until the end. 


%We ask themselves if from a modality the network learns what is more important or more significant w.r.t the other one. 
%In other words, if the modalities representations that each stream learned place the final classifier in "fair" condition i.e. give the opportunity to measure and understand what modality information is really more important.  


%We ask themselves if the network is able to find a measure of correlation of two modalities in order to understand whether one of them is not informative, and eventually which one it should not rely on for the final prediction. 




%coherent contents. %Instead, by not exclusively aligning them, we allow the network to exploit the modality complementarities. 


%In fact, by considering the angle between the two feature vectors as a measure of their correlation, by not constraining the angular distance $\theta$ between the two modality representations we leave the network the possibility to either 


%comparing to angular losses (see Section \ref{angular_losses}), by not constraining the angular distance $\theta$ between the two modality representations, 



    %have the freedom to arrange in non-overlapping configurations. %(Figure ~\ref{fig:OurLoss}-c).
%\end{enumerate}
%\textbf{1)} Since $\lVert{ f_v }\rVert_2$ and $\lVert{ f_a }\rVert_2$ tend to the same value, features norm ranges are encouraged to be comparable, preventing one modality drowning out the other and improving the final classification prediction.
%\textbf{2)} By reducing the norm of the features while learning the feature extractor, the latter is free to choose which are the less/more discriminative information, and lower/rise their norm accordingly, increasing the generalization ability of the model.
%\textbf{3)} Comparing to standard similarity losses, by not constraining the angular distance $\theta$ between the two modality representations, features distributions have the possibility to arrange in non-overlapping configurations, exploiting the complementarity of the two modalities.

%\remove{
%The effects observable at feature-level of the application of our \mylossRna are represented in Figure \ref{fig:OurLoss}. %for better comprehension. 
%In Figure \ref{fig:OurLoss}-a we represent the features distribution learned with standard cross-entropy loss. As it can be seen, the feature norms of the two modalities differ by a $\delta$, meaning that the respective features lie within different ranges which make the two representations hard to compare. The solution proposed by our \mylossRna  corresponds to \textbf{1)}. In Figures \ref{fig:OurLoss}-b and \ref{fig:OurLoss}-c we show the feature representations obtained by minimizing our loss function. The situation depicted in Figure \ref{fig:OurLoss}-b occurs when audio and visual information ``agree" by means of their modality-specific features. %This recalls the ``ideal" alignment condition aimed for by standard similarity losses. 
%The scenario depicted in Figure \ref{fig:OurLoss}-c is the most interesting, since it represents a situation which is not compatible with the aim of standard similarity losses. As stated in \textbf{3)}, our \mylossRna ensures that the modality-specific features are preserved, allowing the final classifier to exploit their complementarity.  }


% Given a visual input $X^v=(x^v_1,...x^v_N)$ and an audio input $X^a=(x^a_1,...x^a_N)$, $x^v_i \in \mathbb{R}^{T\times H\times W}$ denotes the $i$-th visual sample corresponding to a video clip, and $x^a_i \in \mathbb{R}^{T\times H\times W}$ denotes the $i$-th audio sample, represented as a spectrogram image.


\subsection{Extension to Unsupervised Domain Adaptation}\label{dg}
Under this setting, both labelled source data from a single source domain $\mathcal{S}=(\mathcal{S}^v,\mathcal{S}^a)$, and unlabelled target data $\mathcal{T}=(\mathcal{T}^v$, $\mathcal{T}^a)$ are available during training. Figure \ref{fig:architecture} shows the flow of source and target data, indicating with different colors source visual data (green), source audio data (blue) and target data (orange). We denote with $x_{s,i}=(x^v_{s,i},x^a_{s,i})$ and $x_{t,i}=(x^v_{t,i},x^a_{t,i})$ the $i$-th source and target samples respectively.  As it can be seen from Figure \ref{fig:architecture}, both $x^m_{s,i}$ and $x^m_{t,i}$ are fed to the feature extractor $F^m$ of the $m$-th specific modality, shared between source and target, obtaining respectively the features $f_s=(f^v_s,f^a_s)$ and $f_t=(f^v_t,f^a_t)$. In order to consider the contribution of both source and target data during training, we redefine our \mylossRna under the UDA setting as %i as shown in Equations \ref{eq:loss_s_t}, \ref{eq:loss_s_t_1} and \ref{eq:loss_s_t_2}.
\begin{equation}\label{eq:loss_s_t}
    \mathcal{L}_{RNA}=\mathcal{L}^s_{RNA}+\mathcal{L}^t_{RNA} ,
\end{equation}
\begin{equation}\label{eq:loss_s_t_1}
%\label{formula:rna}
    \mathcal{L}_{RNA}=\left(\frac{\EX[h(X^v_{s,i})]}{\EX[h(X^a_{s,i})]} - 1\right)^2
    %\mathcal{L}^s_{RNA}=\frac{1}{N}\frac{\sum_{x^v_{s,i} \in \mathcal{X}^v_s}h(x^v_{s,i})}{\sum_{x^a_{s,i} \in \mathcal{X}^a_s}h(x^a_{s,i})} \rightarrow 1 ,
\end{equation}
\begin{equation}\label{eq:loss_s_t_2}
    \mathcal{L}_{RNA}=\left(\frac{\EX[h(X^v_{t,i})]}{\EX[h(X^a_{t,i})]} - 1\right)^2
    %\mathcal{L}^t_{RNA}=\frac{1}{N}\frac{\sum_{x^v_{t,i} \in \mathcal{X}^v_t}h(x^v_{t,i})}{\sum_{x^a_{t,i} \in \mathcal{X}^a_t}h(x^a_{t,i})} \rightarrow 1 ,
\end{equation}
By minimizing $\mathcal{L}^s_{RNA}$ we benefit from the considerations described in Section \ref{sec:dg}. Also, by minimizing $\mathcal{L}^t_{RNA}$, and thus learning the reweighting between the modalities on the unlabelled data, the encoded features contain useful information which directly enable us to adapt to the target. \mirco{manca una citazione che conferma questo concetto} 

A problem that often occurs with UDA methods is that forcing an alignment between source and target features increases the risk of affecting the discriminative charateristics of the two, and thus destroying the inter-class separability~\cite{pmlr-v97-liu19b}. 
In our UDA setting, by operating on the two domains through separate $\mathcal{L}^s_{RNA}$ and $\mathcal{L}^t_{RNA}$, we mitigate this risk, preserving the discriminative structure of the two.

%The presence of target data during training allows the \mylossRna to benefit from the considerations described in the previous Section \ref{sec:dg} by directly adapting on the unseen domain.








%The RNA loss \mylossRna can be minimized in two ways: either by increasing the $f_v$ norm $(f_v \nearrow)$ or decreasing the $f_a$ norm $(f_a \searrow)$. 

%%DA RIFORMULARE 

%We represent in Figure \ref{fig:OurLoss} an intuition of the feature adjustment behaviour. At the beginning of the training process [Cita Figura 1a!], the feature norms of the two modalities differ by a large $\delta$. By minimizing $\mathcal{L}_{RNA}$, and thus reducing $\delta$ to zero, the network can adjust features distributions in different possible ways, introducing the following advantages.
%(1) It encourages the features norm ranges to be comparable, preventing one modality drowning out the other and improving the final classification prediction [Cita figura 1-b-c!]. (2) By reducing the norm of the features while learning the feature extractor, the latter is free to choose which are the less/more discriminative information, and lower/rise their norm accordingly, increasing the generality of the model. (3) Comparing to standard similarity losses, by not constraining the angular distance $\theta$ between the two modality representations, we leave the features distributions the possibility to arrange in non-overlapping configurations, as in the scenario represented in Figure [Cita Figura 1-c!], exploiting the complementarity of the two modalities.  



%by not constraining the angular distance $\theta$ between the two modality representations, we leave the network the possibility to accentuate the modality-specific features [Cita Figura 1c], allowing them to arrange in an orthogonal scheme which result in a complementarity between the two. 








%we impose a relative alignment between the two modality norms, without constraining the angular distance $\theta$ between the two modality representations.



%Our loss and how it works.
%\subsection{Diamo un nome alla nostra loss!}
%We introduce a new loss function to minimize $\delta$, and defined as:






%If we have a discrepancy between the distributions of the features of the 2 modalities we need a method to balance the two contributions





==> latex/OldFiles/Tabelle_vecchie.tex <==
\begin{table*}
\hfill
\begin{minipage}{0.421\linewidth}

\begin{adjustbox}{width=1\columnwidth, margin=0ex 1ex 0ex 0ex}
\begin{tabular}{lcccc}
\toprule\noalign{\smallskip}
\multicolumn{5}{c}{\normalsize\textsc{Multi Source DG }} \\
\noalign{\smallskip}
\cline{1-5}
\noalign{\smallskip}
  & \multicolumn{1}{c}{D1, D2  $\rightarrow$ D3} & D1, D3  $\rightarrow$ D2 & D2, D3  $\rightarrow$ D1 & Mean\\ 
 \noalign{\smallskip}

\hline
 \noalign{\smallskip}

Deep All      &       51.47                    &   43.19   & 39.35 & 44.67 \\ \hline
 \noalign{\smallskip}

Align. Only       &       50.01                   &   42.40   & 44.40 & 45.60 \\ %\hline
 \noalign{\smallskip}

Orth. Only     &       53.08                  &    41.76  &  48.07 &  47.64\\ %\hline
 \noalign{\smallskip}

BatchNorm     &       52.07                    &   42.63  &  45.14 &  46.61 \\ %\hline
 \noalign{\smallskip}

MM-SADA (Only SS)   \cite{Munro_2020_CVPR}          &       51.87                     &  39.79   & \underline{52.73} & 48.13    \\ 
 \noalign{\smallskip}
\hline


RNA-Net (Ours) &      \underline{55.88}                     &   \underline{45.65}    &   51.64 &  \textbf{51.06} \\ 
\bottomrule
\end{tabular}
\end{adjustbox}

\end{minipage}
\caption{Top-1 Accuracy ($\%$) of our RNA-Net under the single-source DG setting (left) and the multi-source DG setting (right).}
\label{tab:single-source-dg}
\vspace{-0.2cm}
\end{table*}
 

%%% ------------------- UDA table --------------------
\begin{table*}[ht]


\centering
\begin{adjustbox}{width=0.7\columnwidth, margin=0ex 1ex 0ex 0ex}
\begin{tabular}{lccccccc}
\toprule\noalign{\smallskip}
\multicolumn{8}{c}{\normalsize\textsc{UDA }} \\
\noalign{\smallskip}
\cline{1-8}
\noalign{\smallskip}

         & \multicolumn{1}{c}{D1 $\rightarrow$ D2} & D1 $\rightarrow$ D3 & D2  $\rightarrow$ D1 & D2 $\rightarrow$ D3 & D3  $\rightarrow$ D1 & D3  $\rightarrow$ D2    & Mean \\  \hline
         \noalign{\smallskip}

MM-SADA (Only SS) \cite{Munro_2020_CVPR}         &       44.83                   &  42.88     &   40.61   &   \underline{54.21}   &   42.58    &    53.50 & 46.44  \\ %\hline
\noalign{\smallskip}

Adversarial Only \cite{grl-pmlr-v37-ganin15}        &          41.02                  &   43.04     &  39.36     &  49.25      & 38.77      &     50.56     &      43.67     \\ %\hline
\noalign{\smallskip}

MM-SADA \cite{Munro_2020_CVPR}         &         \underline{48.90}                   &  46.66    &  39.51    &   50.89    & \underline{45.42}      &\underline{55.14} & 47.75        \\ %\hline
\noalign{\smallskip}

MMD \cite{da-mmdlong2015learning}         &        42.40                   &  43.84     &  40.87    &  48.13   & 41.46        &50.03  & 44.46        \\ %\hline
\noalign{\smallskip}

AdaBN \cite{ada-bn}         &       36.64                   &  42.57    & 33.97      &   46.63    & 40.51        &  51.20 & 41.92        \\ \hline
\noalign{\smallskip}


RNA-Net (Ours)      &       46.89                  &  48.40   &   41.58   &  51.77    &   43.19    &    54.43 & 47.71  \\ %\hline
\noalign{\smallskip}

RNA-Net+GRL (Ours)      &       46.65                 &  \underline{49.95}   &  \underline{46.06}   &  51.77    &   42.20    &    53.14 & \textbf{48.30 } \\ 

\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Top-1 accuracy ($\%$) of our RNA-Net under the multi-modal UDA setting.}
\label{tab:multi-modal-da}
\vspace{-0.3cm}

\end{table*}
\noindent

==> latex/OldFiles/oldMethod.tex <==
\subsection{Intuition and Motivation}

A common strategy in the literature is to tackle the first person action recognition task using a multi-modal approach~\cite{Munro_2020_CVPR,Kazakos_2019_ICCV,lin2019tsm,cartas2019seeing,kazakos2021slow,wang2016temporal}. 
However, as the number of parameters to train increases, the network tends to overfit, restricting the network's generability on target and resulting in a noticeable drop in performance when compared to the best uni-modal solution~\cite{gradient-blending,alamri2019audio,goyal2017making,poliak2018hypothesis,weston2011wsabie}. In particular, authors of~\cite{gradient-blending} %brought to light that different modalities overfit and generalize at different rates, so training them jointly with a single optimization strategy could be sub-optimal. 
%They 
formalized the phenomenon through the overfitting-to-generalization ratio ($OGR$) metric. 
The solution proposed in~\cite{gradient-blending} is based on a re-weighting of the different modalities with an appropriate phase of estimating-weights that aims to minimize ${OGR}^2$. 

\begin{figure}[t]
    %\includegraphics[width=1\linewidth]{latex/Img/qualitative.png}
    \includegraphics[width=0.97\linewidth]{latex/Img/Plot_WACV_2.pdf}
     %\includegraphics[width=1\linewidth]{latex/Img/Qualitative_3.pdf}
    \caption{By training both streams jointly, and testing on separate ones, the RGB performance drop consistently (left). This drop in performance is due to an “unbalance" at feature-norm level which, when mitigated, leads to better performance (right).} 
    %We show one case where the RGB modality provides a correct prediction after norm re-balance.} %In the first case (\textbf{top}), the RGB modality leads to the final prediction, while in the second one (\textbf{bottom}) the audio modality leads.  }
    \label{fig:norm_ranges}
 %   \vspace{-0.3cm}
\end{figure} 
Although the weights are dependant of the task and dataset, the fact that each modality requires a different weight suggested us that the network considers one modality to be more convenient to utilize in solving the task and prefers it in the final prediction.
Motivated by these findings, we empirically measured the negative effects of this phenomenon in our context, both training and test time. As illustrated in Figure \ref{fig:norm_ranges}-a, when training RGB and audio streams separately, both modalities perform equally well, as can be observed. When training together, however, the RGB accuracy drops consistently at test time. Surprisingly, the accuracy of the audio modality seems not to be affected. 


Our intuition is that an “unbalance" exists between the two modalities during training, which prevents the network to learn “equally” from the two. Specifically, we believe that \textit{the network tends to “privilege” one modality over the other during training, while “penalising” the other.} We also wondered if this concept, i.e., the unbalance that arises between the modalities during the training phase, could be extended to a multi-source context.
Is it possible that one source has a greater influence on the other, causing the final model to be influenced negatively?
Starting from the above considerations, we sought a function that captures the amount of information contained in the final embedding of each modality and possibly highlights the presence of this unbalance.  %during training. 
Our objective is thus to find an appropriate loss which is able to induce a re-balance not only between the various modality, but also between the input sources.


Several works have highlighted the existence of a strong correlation between the \textit{mean feature norm} and the amount of “valuable" information for classification~\cite{zheng2018ring,wang2017normface,ranjan2017l2}. The cross-entropy loss, in particular, is demonstrated to encourage well-separated features with a high norm value in~\cite{wang2017normface}. Indeed, authors of~\cite{zheng2018ring} showed that low norm features have huge variation in angular classification margin, which translates to higher errors in classification. 
Motivated by these findings, we chose the $L2$-norm of the feature descriptor as a metric for assessing the imbalance between the two training modalities, as it has been proven to be indicative of their informative content. As evidence of this, Figure \ref{fig:norm_ranges}-b shows that the modality with the greatest norm (audio) dominates the learning of the RGB one negatively affecting the performance. This observation is also supported by the Smaller-Norm-Less-Informative assumption~\cite{ye2018rethinking}, which suggests that the modality representation with the smaller norm is less informative during inference. Motivated by these findings, we propose a simple yet effective loss whose goal is to re-balance the mean feature modality norms during training, allowing the network to fully exploit joint training, especially in cross-domain scenarios. 


==> latex/OldFiles/otherLoss.tex <==
\begin{table}
 \begin{minipage}[t]{\linewidth}
 \centering


\setlength{\tabcolsep}{2pt}
\begin{adjustbox}{width=0.6\linewidth}
\begin{tabular}{lcccc}
\toprule\noalign{\smallskip}
%
Method & Single-DG & Multi-DG & Norm & Angle\\
 \noalign{\smallskip} \hline \noalign{\smallskip}
 Source-Only & 41.87 & 44.67 & &\\       
\hline
 \noalign{\smallskip}

CosSim & 41.76 & 45.60 & & \checkmark \\
MSE & 45.52 & 46.11   & \checkmark  & \checkmark  \\ %\hline
Orth.Loss & 42.67 & 47.64   &&\checkmark    \\ %\hline
 \noalign{\smallskip}

\hline \noalign{\smallskip}

RNA-Net & \textbf{45.75} & \textbf{51.06} & \checkmark &     \\ %\hline
\bottomrule
\end{tabular}
\end{adjustbox}
\end{minipage}
\caption{Placeholder}
\end{table}


==> latex/SuppMat/FusionStrategy.tex <==
\textbf{Fusion Strategies.} %To verify the effectiveness of our design choice, we introduce a loss variant, called \textit{Hard Norm Alignment} (HNA), that induces the norms to tend to a given value arbitrarily $R$. The $R$ term is chosen after observing the range of the norms of the two modalities, and picking a value half-way between the two. 
In Table \ref{tab:ablations} we compare the \textit{late fusion} approach against the so-called \textit{mid-level fusion}, used in \cite{Kazakos_2019_ICCV}. %It consists in feeding the prediction layer with the fusion of the two modality features, i.e., concatenation.
It consists in feeding the prediction layer a concatenation of the two modality features.
%The results are shown . % Note how HNA performs worse than $\mathcal{L}_{RNA}$ in all contexts, confirming that an ``hard'' loss function constitutes in a limit. %Instead, letting the proportion between the norms of the two self-reweighting by our $\mathcal{L}_{RNA}$ leads to better results (up to $1\%$). 
As far as it concerns the mid-level fusion approach, it demonstrates to be a valid alternative in both the intra-domain (\textit{Supervised}) and cross-domain scenarios, remarking the flexibility of our method to be employed with different multi-modal fusion strategies and in all the presented settings. %It has to be noticed that RNA-Net achieves good performance also intra-domain (\textit{Supervised}).

\input{latex/Tables/Ablation}


==> latex/Tables/Ablation.tex <==
\begin{table}
\centering

\begin{adjustbox}{width=1.0\columnwidth, margin=0ex 1ex 0ex 0ex}
\begin{tabular}{l|cccc}


\toprule\noalign{\smallskip}
\multicolumn{5}{c}{\normalsize\textsc{Fusion strategies}} \\
\noalign{\smallskip}
\cline{1-5}
\noalign{\smallskip}
  & \multicolumn{1}{c}{Supervised} & Single-DG & Multi-DG & DA\\ 
 \noalign{\smallskip} \hline
 \noalign{\smallskip}


Baseline (\textit{mid-level fusion})    & 60.18          & 40.33          & 47.61          & 40.33               \\
RNA-Net (\textit{mid-level fusion})  & 62.11          & 45.48          & 49.56          & 45.73           \\

\hline
 \noalign{\smallskip}
Baseline (\textit{late fusion})  & 59.76          & 40.93          & 44.67          & 40.93               \\


RNA-Net  (\textit{late fusion})      & \textbf{63.13} & \textbf{45.75} & \textbf{51.06} & \textbf{47.71}  \\
\bottomrule

\end{tabular}
\end{adjustbox}
\caption{Top-1 Accuracy ($\%$) of RNA-Net with two different fusion strategies, namely \textit{mid-level fusion} and \textit{late fusion}. \textbf{Bold:} highest result for each setting. }
\label{tab:ablation_}
\end{table}


==> latex/Tables/Ablation2.tex <==
% \usepackage{multirow}


\begin{table}
\centering


\begin{tabular}{l|lr}
\multicolumn{2}{l}{Ablations}                     & \multicolumn{1}{l}{Mean}  \\ \hline \hline
\multirow{4}{*}{Baseline} & Supervised Target & 59,76                     \\
                             & Source Only       & 40,93               \\
                             & Deep All          & 44,67                    \\ \hline
\multirow{4}{*}{HNA}         & Supervised Target & 62,41               \\
                             & DG                & 44,58               \\
                             & Multi DG          & 46,7     \\ 
                             & DA                & 47,19             \\ \hline
\multirow{4}{*}{RNA}         & Supervised Target & 63,13               \\
                             & DG                & 45,75                   \\
                             & Multi DG          & 51,06               \\ 
                             & DA                & 47,71      \\ \hline
\multirow{4}{*}{Fusion}      & Supervised Target & 60,18                     \\ 
                             & Source Only       & 40,33               \\
                             & Deep All          & 47,61      
                                         \\ \hline
\multirow{4}{*}{RNA - Fusion}  & Supervised Target & 62,11               \\
                             & DG                & 45,48               \\
                             & Multi DG          & 49,56      \\ 
                             & DA                & 45,73                  \\  \hline
\end{tabular}
\end{table}

==> latex/Tables/Flow.tex <==
\begin{table}
\centering

\begin{adjustbox}{width=1.0\columnwidth, margin=0ex 1ex 0ex 0ex}
\begin{tabular}{l|cccc}


\toprule\noalign{\smallskip}
\multicolumn{5}{c}{\normalsize\textsc{RGB+Audio+\textbf{Flow}}} \\
\noalign{\smallskip}
\cline{1-5}
\noalign{\smallskip}
  & \multicolumn{1}{c}{D1, D2 $\rightarrow$ D3} & D1, D3 $\rightarrow$ D2 & D2, D3 $\rightarrow$ D1 & Mean\\ 
 \noalign{\smallskip} \hline
 \noalign{\smallskip}


Baseline    & 54.65	&	45.29	&	44.46	&	48.13               \\
RNA-Net   & 56.63	&	47.87	&	53.65 &	\textbf{52.72}         \\


\bottomrule

\end{tabular}
\end{adjustbox}
\caption{Top-1 Accuracy ($\%$) of RNA-Net extended with Flow modality. }
\label{tab:ablation_}
\end{table}


==> latex/Tables/LossComparison.tex <==
\begin{table}
 \begin{minipage}[t]{\linewidth}
 \centering

\begin{adjustbox}{width=0.85\linewidth}
\begin{tabular}{lccccc}
\toprule\noalign{\smallskip}
%\multicolumn{6}{c}{\normalsize\textsc{Comparison with other losses }} \\
%\noalign{\smallskip}
%\cline{1-6}
%\noalign{\smallskip}
           & Source-Only & Cos Sim & MSE & Orth Lss & RNA            \\ \hline
 %\noalign{\smallskip} \hline \noalign{\smallskip}
 Angle  &  & \checkmark & \checkmark & \checkmark &  \\      
% \noalign{\smallskip}
 Magnitude  &  &  & \checkmark &  & \checkmark \\
\hline
% \noalign{\smallskip}

Single DG & 41.87       & 41.76   & 45.52        & 42.67    & \textbf{45.75} \\
Multi-DG & 44.67       & 45.60   & 46.11        & 47.64    & \textbf{51.06} \\ %\hline
 %\noalign
\bottomrule
\end{tabular}
\end{adjustbox}
\end{minipage}
\caption{Placeholder}
\end{table}



==> latex/Tables/multi-modal-da.tex <==
\begin{table*}[thb!]
\centering
\begin{adjustbox}{width=0.7\columnwidth, margin=0ex 1ex 0ex 0ex}
\begin{tabular}{l|cccccc|c}
\hline \hline
Multi-Modal                & \multicolumn{1}{c}{D1 $\rightarrow$ D2} & D1 $\rightarrow$ D3 & D2  $\rightarrow$ D1 & D2 $\rightarrow$ D3 & D3  $\rightarrow$ D1 & D3  $\rightarrow$ D2    & Mean \\ \hline \hline
SS Only         &       44,83                   &  42,88     &   40,61   &   54,21   &   42,58    &    53,5 & 46,44  \\ %\hline
Adversarial Only         &          41,02                  &   43,04     &  39,36     &  49,25      & 38,77      &     50,56     &      43,67     \\ %\hline
MMSADA \cite{Munro_2020_CVPR}         &         48,9                   &  46,66    &  39,51    &   50,89    & 45,42      &55,14 & 47,75        \\ %\hline
MMD \cite{da-mmdlong2015learning}         &        42,4                   &  43,84     &  40,87    &  48,13   & 41,46        &50,03  & 44,46        \\ %\hline
AdaBN \cite{ada-bn}         &       36,64                   &  42,57    & 33,97      &   46,63    & 40,51        &  51,2 & 41,92        \\ \hline

RNA  (Ours)      &       46,89                  &  48,4   &   41,58   &  51,77    &   43,19    &    54,43 & 47,71  \\ %\hline
RNA + GRL (Ours)      &       \underline{47,54}                 &  47,71   &  43,19   &  52,83    &   43,02    &    54,1 & \textbf{48,07 } \\ \hline


\end{tabular}
\end{adjustbox}
\caption{}
\label{tab:multi-modal-da}

\end{table*}


==> latex/Tables/multi-source-dg.tex <==
\begin{table}[t]
\begin{adjustbox}{width=1.0\columnwidth, margin=0ex 1ex 0ex 0ex}
\begin{tabular}{lccccccc}
\hline \hline
Multi-Source  & \multicolumn{1}{c}{D1, D2  $\rightarrow$ D3} & D1, D3  $\rightarrow$ D2 & D2, D3  $\rightarrow$ D1 & Mean\\ \hline
Deep All      &       51,47                    &   43,19   & 39,35 & 44,67 \\ \hline
AlignLoss       &       50,01                   &   42,4   & 44,4 & 45,6 \\ \hline
OrthLoss     &       53,08                  &    41,76  &  48,07 &  47,64\\ \hline
Norm     &       52,07                    &   42,63  &  45,14 &  46,61 \\ \hline
SS            &       51,87                     &  39,79   & 52,73 & 48,13    \\ \hline
RNA (Ours) &      55,88                     &   45,65    &   51,64 &  \textbf{51,06} \\ \hline 
\hline
\end{tabular}
\end{adjustbox}
\caption{}
\label{tab:multi-source-dg}

\end{table}


==> latex/Tables/single-modality.tex <==
\begin{table*}[hbt!]
\begin{tabular}{lccccccc}
\hline \hline
           & \multicolumn{1}{c}{D1 $\rightarrow$ D2} & D1 $\rightarrow$ D3 & D2 $\rightarrow$ D1     & D2 $\rightarrow$ D3     & D3 $\rightarrow$ D1     & D3 $\rightarrow$ D2   & Mean  \\ \hline
Source Only (RGB) &      34,15                      &    35,03  &     34,76    &  38,79       &      33,03    &    41,08     &  36,14  \\ \hline
Source Only (Audio) &     31,90                      &   36,49    &   29,17       &   44,00       &     34,00    &  42,93 & 36,42        \\ \hline
Source Only (RGB+Audio) &    39,03&	39,17	&35,27&	47,52&	40,26&	49,98&	41,87       \\ \hline
\hline
Supervised (RGB) & \multicolumn{2}{c}{51,72}              & \multicolumn{2}{c}{61,65} & \multicolumn{2}{c}{60,37} & 57,91 \\ \hline 

Supervised (Audio) & \multicolumn{2}{c}{45,24}              & \multicolumn{2}{c}{58,83} & \multicolumn{2}{c}{61,56} & 55,21\\ \hline 

Supervised (RGB+Audio)  & \multicolumn{2}{c}{50,30}              & \multicolumn{2}{c}{64,40} & \multicolumn{2}{c}{63,50} & \textbf{59,40}\\ \hline \hline
\end{tabular}
\caption{Top-1 accuracy of (nome dell'esperimento. Single modality non so se e' corretto visto che abbiamo anche il multi). Source Only: train on source $\mathcal{S}$ and test on target $\mathcal{T}$ ($\mathcal{S}$ $\rightarrow$ $\mathcal{T}$). Supervised: train and test on $\mathcal{T}$ ($\mathcal{T}$ $\rightarrow$ $\mathcal{T}$)}
\label{tab:single-mod}

\end{table*}

==> latex/Tables/single-source-dg.tex <==
\begin{table}[t]
\begin{adjustbox}{width=1.0\columnwidth, margin=0ex 1ex 0ex 0ex}
\begin{tabular}{l|cccccc|c}
\toprule\noalign{\smallskip}

% OPPURE
%\begin{tabularx}{\columnwidth}{X|XXXXXXX}

\hline

             & \multicolumn{1}{c}{D1 $\rightarrow$ D2} & D1 $\rightarrow$ D3 & D2  $\rightarrow$ D1     & D2 $\rightarrow$  D3     & D3  $\rightarrow$ D1     & D3  $\rightarrow$ D2   & Mean   \\ \hline
Source Only &    39,03&	39,17	&35,27&	47,52&	40,26&	49,98&	41,87  \\ \hline \hline
AlignLoss   &    38,50                        &   33,75    &     32,59       &    45,78       &    39,97       &      50,86 & 41,76     \\ \hline
OrthLoss     &    39,18                        &    37,55    &      36,86      &     47,09      &      43,70    &       51,61   & 42,67 \\ \hline
Norm    &   40,03                        &    39,88    &      36,39      &    48,47     &     42,60     &      48,33    & 42,62 \\ \hline
SS   &    38,86                        &    33,75   &      32,59      &     45,78     &       39,97     &       50,86    & 40,30 \\ \hline

RNA (Ours) &      45,01                      &  44,62   &    41,76     &    48,90       &       42,20  &    51,98 & \textbf{45,75}       \\ \hline

\hline

%\end{tabularx}

\end{tabular}
\end{adjustbox}

\caption{Top-1 accuracy of multi-modal single-source domain generalization setting.}
\label{tab:single-source-dg}
\end{table}

==> latex/Tables/tbn-fusion.tex <==
\begin{table*}[hbt!]
\begin{tabular}{lcccccc}
\hline
\hline
Fusion             & \multicolumn{1}{c}{D1 $\rightarrow$ D2} & D1 $\rightarrow$ D3 & D2  $\rightarrow$ D1     & D2  $\rightarrow$  D3     & D3  $\rightarrow$ D1     & D3  $\rightarrow$ D2     \\ \hline

\hline
TBN (Source Only) &                           &       &           &           &           &           \\ \hline
TBN (DG) &                            &       &           &           &           &           \\ \hline
TBN (DA) &                            &       &           &           &           &           \\ \hline
TBN Supervised &                            &       &           &           &           &           \\ \hline \hline
Ours RELATIVE Fusion (Source Only) &     \checkmark                       &    \checkmark   &     \checkmark      &    \checkmark       &      \checkmark     &      \checkmark     \\ \hline
Ours RELATIVE Fusion (DG) &     \checkmark                       &     \checkmark  &    \checkmark       &    \checkmark       &       \checkmark    &     \checkmark      \\ \hline

Ours RELATIVE + GRL Fusion (DA) &                       \checkmark   &  \checkmark     &     \checkmark      &   \checkmark        &   \checkmark        &     \checkmark      \\ \hline

Supervised Fusion   & \multicolumn{2}{c}{\checkmark}              & \multicolumn{2}{c}{\checkmark} & \multicolumn{2}{c}{\checkmark} \\ \hline \hline
\end{tabular}
\caption{}

\end{table*}
